As Advertised? Understanding the Impact of Influencer VPN Ads

Influencer VPN ads (sponsored segments) on YouTube often disseminate misleading information about both VPNs, and security & privacy more broadly. However, it remains unclear how (or whether) these ads affect users' perceptions and knowledge about VPNs. In this work, we explore the relationship between YouTube VPN ad exposure and users' mental models of VPNs, security, and privacy. We use a novel VPN ad detection model to calculate the ad exposure of 217 participants via their YouTube watch histories, and we develop scales to characterize their mental models in relation to claims commonly made in VPN ads. Through (pre-registered) regression-based analysis, we find that exposure to VPN ads is significantly correlated with familiarity with VPN brands and increased belief in (hyperbolic) threats. While not specific to VPNs, these threats are often discussed in VPN ads. In contrast, although many participants agree with both factual and misleading mental models of VPNs that often appear in ads, we find no significant correlation between exposure to VPN ads and these mental models. These findings suggest that, if VPN ads do impact mental models, then it is predominantly emotional (i.e., threat perceptions) rather than technical.

==> intro.tex <==
\section{Introduction}

People are often called on to make decisions that affect their 
digital \sp---e.g., about what software or platforms to use or what 
information to share in different contexts.
%
How a user reacts to these decisions depends not only on their preferences
and values, but on their understanding of the threats they face and the
capabilities of any proactive measures they are considering.
%
A user with misaligned mental models of threats or capabilities may
inadvertently expose themselves to threats, or experience undue hardship
while implementing redundant protections.
%
Because of this, researchers have long studied users to identify (and
suggest ways to improve) misaligned mental models of \sp 
tools~\cite{ruba2017obstacles, ruba2018e2ee, 
christian2021e2ee, krombholz2019if, dechand2019encryption, 
wu2018tree, bai2020improving, akgul2021evaluating}. 


An adjacent body of work investigates how users learn about \sp,
how their \sp mental models form, and where users find \sp advice.
%
Researchers have demonstrated influence from many sources, including media 
depictions, family and friends, personal research and experiences, experts, 
social media, formal education, and work-based training~\cite{fulton2019media, 
redmiles2016learn, baig2021media, tahaei2021don, redmiles2016think, 
namara2020emotional}, with media depictions often reported as the top 
source~\cite{redmiles2016learn, routi2017posture}.
%
Most of these findings are based on self-report data which, while valuable, 
is subject to important limitations in what participants can recall and 
articulate.


In this work, we take a first step towards addressing those limitations:
we investigate the correlation between mental models of \sp and 
\textit{measured exposure} to relevant media, using \textit{influencer VPN ads} 
on YouTube (\vpnads) as an exemplar.
%
We focus on VPN ads for two main reasons.


First, \vpnads are a recent but prominent form of \sp media that may have
substantial impact on users' \sp postures.
%
Prior work found that advertisements directly embedded in videos by content 
creators (\yters), which sometimes receive millions of views, are often vague 
and include misleading information about the protections that VPNs can 
provide~\cite{akgul2022vpn}.
%
These \vpnads also often describe internet threats in broad terms outside
the context of VPNs, and therefore have the potential to influence both
users' specific mental models of VPNs, and their general mental models
of \sp.
%
\vpnads make an excellent target for out investigation, as their content
has been thoroughly documented and characterized, but their actual effect on
users' mental models remains unclear.


Second, as we will demonstrate in this work, exposure to \vpnads 
can be measured with relatively few confounds compared to other forms
of media exposure. 

%Further, despite being repeatedly found as the top influencing factor, 
%the effect of media on mental models is still 
%only based on self-report data: 
%participants report where they remember learning from. This type of 
%data is necessary in research but is subject to serious limitations.

%More recently, an unexpected (potential) influence on mental models 
%have been found in the form of \textit{influencer 
%VPN ads} (\vpnads)~\cite{akgul2022vpn}.
%These ads, directly embedded in videos 
%by content creators (\yters), are often 
%vague and can mislead users about what VPNs can provide. 
%More alarmingly, \vpnads have been found to advertise threat models 
%independent of VPNs, potentially leading to an influence 
%on \sp mental models at a larger scale.
%Despite speculation, 
%the exact effects of \vpnads on users, if any, remains unclear.

%Our work takes a first step to address these shortcomings, 
%we are the first to attempt to show a 
%correlation between mental models of \sp and 
%\textit{real world exposure} to \sp media through the world of \vpnads.

%This study focuses on \vpnads due to four primary 
%reasons: (1) \vpnads are a recent but 
%prominent form of \sp media; (2) they have been 
%formally measured and characterized, we know what 
%to expect from them; (3) \vpnads are often misleading 
%and might have serious implications on users' 
%\sp posture; and (4) we demonstrate that exposure to \vpnads can be 
%measured with relatively few confounds.

We present a novel, multi-stage user study design with which we gather
not only participants' mental models, but also \emph{their entire \yt
viewing history}.
%
These rich datasets allow us to not just rely on self-report data, but
to directly measure the extent to which ad exposure is correlated with
their VPN mental models.
%
More specifically, we address the following four research questions:
%% In this paper, we address the following 4 research questions.
%
%% We use the first question as a baseline to test our methods, and use those
%% methods to answer the 3 subsequent questions:

\smallskip

\begin{itemize}[itemsep=0pt, left=0pt]
    \item \textbf{RQ0:} Does exposure to \vpnads correlate with VPN brand familiarity? 
    \item \textbf{RQ1:} Does exposure to \vpnads correlate with mental models of VPNs?
    \item \textbf{RQ2:} Does exposure to \vpnads correlate with mental models of internet threats?
    \item \textbf{RQ3:} What are the most common threats people believe VPNs protect against? Do people's beliefs mirror findings from prior work on \vpnads?
\end{itemize}

\medskip \noindent
%
We follow a two-step process to answer these questions: an initial exploratory
phase (in which we pilot our data collection approach and form an analysis 
plan), and a final data collection and analysis phase.
%
Mental models were captured through the use of two questionnaires developed
for this work; we define exposure to \vpnads as a logarithmic function of
the total amount of words a participant has seen in \vpnads, measured
using a BERT-based model that analyzes transcripts of participants' \yt
watch histories.
%
With our final instrumentation, we collected mental models, real-world
exposure to \vpnads, and other relevant characteristics for 217 \yt users.


We find significant correlations between exposure to \vpnads, and both
VPN brand familiarity, and belief in threat models commonly advertised in
\vpnads.
%
However, we find no such relationship between exposure to \vpnads and
belief in specific factual or misleading claims about VPN capabilities (common claims in \vpnads).
%
Qualitative analysis of our data suggests that users share similar, but not
identical, mental models to those disseminated through \vpnads.


These findings suggest that \vpnads have a significant impact on mental models
but are more effective at conveying threats than technical details, perhaps
due to emotional appeals associated with threats~\cite{akgul2022vpn, 
obermiller2005ad}.
%
Increased concern about often unrealistic threats might cause unnecessary stress on
users, which might be alleviated by less hyperbolic threat modeling in \vpnads.


%The rest of this section is organized as follows: we discuss related works 
%and backgournd \autoref{sec:related}, describe our 
%methods (\autoref{sec:methods}), and outline our results (\autoref{sec:results}). 
%Implications of our work are given in~\autoref{sec:discussion}.


